Deep Multimodal Guidance for Medical Image Classification

Medical imaging is a cornerstone of therapy and diagnosis in modern medicine. However, the choice of imaging modality for a particular theranostic task typically involves trade-offs between the feasibility of using a particular modality (e.g., short wait times, low cost, fast acquisition, reduced radiation/invasiveness) and the expected performance on a clinical task (e.g., diagnostic accuracy, efficacy of treatment planning and guidance). In this work, we aim to apply the knowledge learned from the less feasible but better-performing (superior) modality to guide the utilization of the more-feasible yet under-performing (inferior) modality and steer it towards improved performance. We focus on the application of deep learning for image-based diagnosis. We develop a light-weight guidance model that leverages the latent representation learned from the superior modality, when training a model that consumes only the inferior modality. We examine the advantages of our method in the context of two clinical applications: multi-task skin lesion classification from clinical and dermoscopic images and brain tumor classification from multi-sequence magnetic resonance imaging (MRI) and histopathology images. For both these scenarios we show a boost in diagnostic performance of the inferior modality without requiring the superior modality. Furthermore, in the case of brain tumor classification, our method outperforms the model trained on the superior modality while producing comparable results to the model that uses both modalities during inference.

==> old_refs.tex <==
@article{survey5,
  title={A survey on deep multimodal learning for computer vision: advances, trends, applications, and datasets},
  author={Bayoudh, Khaled and Knani, Raja and Hamdaoui, Fay{\c{c}}al and Mtibaa, Abdellatif},
  journal={The Visual Computer},
  pages={1--32},
  year={2021},
  publisher={Springer}
}

@article{survey1,
  title={Multimodal machine learning: A survey and taxonomy},
  author={Baltru{\v{s}}aitis, Tadas and Ahuja, Chaitanya and Morency, Louis-Philippe},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={41},
  number={2},
  pages={423--443},
  year={2018},
  publisher={IEEE}
}

@article{survey2,
  title={Deep multimodal representation learning: A survey},
  author={Guo, Wenzhong and Wang, Jianwen and Wang, Shiping},
  journal={IEEE Access},
  volume={7},
  pages={63373--63394},
  year={2019},
  publisher={IEEE}
}

@article{survey4,
  title={Deep multimodal fusion for semantic image segmentation: A survey},
  author={Zhang, Yifei and Sidib{\'e}, D{\'e}sir{\'e} and Morel, Olivier and M{\'e}riaudeau, Fabrice},
  journal={Image and Vision Computing},
  volume={105},
  pages={104042},
  year={2021},
  publisher={Elsevier}
}

@article{survey3,
  title={A survey on deep learning for multimodal data fusion},
  author={Gao, Jing and Li, Peng and Chen, Zhikui and Zhang, Jianing},
  journal={Neural Computation},
  volume={32},
  number={5},
  pages={829--864},
  year={2020},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}

@article{aq1,
  title={A combined PET/CT scanner for clinical oncology},
  author={Beyer, Thomas and Townsend, David W and Brun, Tony and Kinahan, Paul E and Charron, Martin and Roddy, Raymond and Jerin, Jeff and Young, John and Byars, Larry and Nutt, Ronald},
  journal={Journal of nuclear medicine},
  volume={41},
  number={8},
  pages={1369--1379},
  year={2000},
  publisher={Soc Nuclear Med}
}

@article{aq2,
  title={Simultaneous PET and MR imaging},
  author={Shao, Yiping and Cherry, Simon R and Farahani, Keyvan and Meadors, Ken and Siegel, Stefan and Silverman, Robert W and Marsden, Paul K},
  journal={Physics in Medicine \& Biology},
  volume={42},
  number={10},
  pages={1965},
  year={1997},
  publisher={IOP Publishing}
}

@article{pg1,
  title={Glioblastoma: pathology, molecular mechanisms and markers},
  author={Aldape, Kenneth and Zadeh, Gelareh and Mansouri, Sheila and Reifenberger, Guido and von Deimling, Andreas},
  journal={Acta neuropathologica},
  volume={129},
  number={6},
  pages={829--848},
  year={2015},
  publisher={Springer}
}

@article{pg2,
  title={Using the molecular classification of glioblastoma to inform personalized treatment},
  author={Olar, Adriana and Aldape, Kenneth D},
  journal={The Journal of pathology},
  volume={232},
  number={2},
  pages={165--177},
  year={2014},
  publisher={Wiley Online Library}
}

@article{ct,
  title={Patients undergoing recurrent CT scans: assessing the magnitude},
  author={Rehani, Madan M and Yang, Kai and Melick, Emily R and Heil, John and {\v{S}}al{\'a}t, Du{\v{s}}an and Sensakovic, William F and Liu, Bob},
  journal={European radiology},
  volume={30},
  number={4},
  pages={1828--1836},
  year={2020},
  publisher={Springer}
}

@article{biopsy,
  title={Systematic review of complications of prostate biopsy},
  author={Loeb, Stacy and Vellekoop, Annelies and Ahmed, Hashim U and Catto, James and Emberton, Mark and Nam, Robert and Rosario, Derek J and Scattoni, Vincenzo and Lotan, Yair},
  journal={European urology},
  volume={64},
  number={6},
  pages={876--892},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{medmm,
  title={Deep learning in multimodal medical image analysis},
  author={Xu, Yan},
  booktitle={International Conference on Health Information Science},
  pages={193--200},
  year={2019},
  organization={Springer}
}

@article{inputfusion1,
  title={Context aware deep learning for brain tumor segmentation, subtype classification, and survival prediction using radiology images},
  author={Pei, Linmin and Vidyaratne, Lasitha and Rahman, Md Monibor and Iftekharuddin, Khan M},
  journal={Scientific Reports},
  volume={10},
  number={1},
  pages={1--11},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{inputfusion2,
  title={Deep learning-based image segmentation on multimodal medical imaging},
  author={Guo, Zhe and Li, Xiang and Huang, Heng and Guo, Ning and Li, Quanzheng},
  journal={IEEE Transactions on Radiation and Plasma Medical Sciences},
  volume={3},
  number={2},
  pages={162--169},
  year={2019},
  publisher={IEEE}
}

@article{pathomic,
  title={Pathomic fusion: an integrated framework for fusing histopathology and genomic features for cancer diagnosis and prognosis},
  author={Chen, Richard J and Lu, Ming Y and Wang, Jingwen and Williamson, Drew FK and Rodig, Scott J and Lindeman, Neal I and Mahmood, Faisal},
  journal={IEEE Transactions on Medical Imaging},
  year={2020},
  publisher={IEEE}
}

@inproceedings{mmo,
  title={Deep orthogonal fusion: Multimodal prognostic biomarker discovery integrating radiology, pathology, genomic, and clinical data},
  author={Braman, Nathaniel and Gordon, Jacob WH and Goossens, Emery T and Willis, Caleb and Stumpe, Martin C and Venkataraman, Jagadish},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={667--677},
  year={2021},
  organization={Springer}
}

@article{sevenpt,
  title={Seven-point checklist and skin lesion classification using multitask multimodal neural nets},
  author={Kawahara, Jeremy and Daneshvar, Sara and Argenziano, Giuseppe and Hamarneh, Ghassan},
  journal={IEEE journal of biomedical and health informatics},
  volume={23},
  number={2},
  pages={538--546},
  year={2018},
  publisher={IEEE}
}

@article{ensemble,
  title={An ensemble of fine-tuned convolutional neural networks for medical image classification},
  author={Kumar, Ashnil and Kim, Jinman and Lyndon, David and Fulham, Michael and Feng, Dagan},
  journal={IEEE journal of biomedical and health informatics},
  volume={21},
  number={1},
  pages={31--40},
  year={2016},
  publisher={IEEE}
}

@article{concat1,
  title={Predicting cancer outcomes from histology and genomics using convolutional networks},
  author={Mobadersany, Pooya and Yousefi, Safoora and Amgad, Mohamed and Gutman, David A and Barnholtz-Sloan, Jill S and Vega, Jos{\'e} E Vel{\'a}zquez and Brat, Daniel J and Cooper, Lee AD},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={13},
  pages={E2970--E2979},
  year={2018},
  publisher={National Acad Sciences}
}

@article{radpath,
  title={Segmentation and classification in digital pathology for glioma research: challenges and deep learning approaches},
  author={Kurc, Tahsin and Bakas, Spyridon and Ren, Xuhua and Bagari, Aditya and Momeni, Alexandre and Huang, Yue and Zhang, Lichi and Kumar, Ashish and Thibault, Marc and Qi, Qi and others},
  journal={Frontiers in neuroscience},
  pages={27},
  year={2020},
  publisher={Frontiers}
}

@article{checklist,
  title={Epiluminescence microscopy for the diagnosis of doubtful melanocytic skin lesions: comparison of the ABCD rule of dermatoscopy and a new 7-point checklist based on pattern analysis},
  author={Argenziano, Giuseppe and Fabbrocini, Gabriella and Carli, Paolo and De Giorgi, Vincenzo and Sammarco, Elena and Delfino, Mario},
  journal={Archives of dermatology},
  volume={134},
  number={12},
  pages={1563--1570},
  year={1998},
  publisher={American Medical Association}
}

@inproceedings{radpath_winners,
  title={Brain tumor classification with multimodal MR and pathology images},
  author={Ma, Xiao and Jia, Fucang},
  booktitle={International MICCAI Brainlesion Workshop},
  pages={343--352},
  year={2019},
  organization={Springer}
}

@article{CLAM,
  title={Data-efficient and weakly supervised computational pathology on whole-slide images},
  author={Lu, Ming Y and Williamson, Drew FK and Chen, Tiffany Y and Chen, Richard J and Barbieri, Matteo and Mahmood, Faisal},
  journal={Nature biomedical engineering},
  volume={5},
  number={6},
  pages={555--570},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{metrics,
  title={Metrics for multi-class classification: an overview},
  author={Grandini, Margherita and Bagli, Enrico and Visani, Giorgio},
  journal={arXiv preprint arXiv:2008.05756},
  year={2020}
}

@article{st,
  title={Knowledge distillation and student-teacher learning for visual intelligence: A review and new outlooks},
  author={Wang, Lin and Yoon, Kuk-Jin},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2021},
  publisher={IEEE}
}

@inproceedings{audiovideo2,
  title={Emotion recognition in speech using cross-modal transfer in the wild},
  author={Albanie, Samuel and Nagrani, Arsha and Vedaldi, Andrea and Zisserman, Andrew},
  booktitle={Proceedings of the 26th ACM international conference on Multimedia},
  pages={292--301},
  year={2018}
}

@inproceedings{audiovideo1,
  title={Asr is all you need: Cross-modal distillation for lip reading},
  author={Afouras, Triantafyllos and Chung, Joon Son and Zisserman, Andrew},
  booktitle={ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={2143--2147},
  year={2020},
  organization={IEEE}
}

@inproceedings{audiovideo3,
  title={Seeing voices and hearing faces: Cross-modal biometric matching},
  author={Nagrani, Arsha and Albanie, Samuel and Zisserman, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={8427--8436},
  year={2018}
}

@article{medst1,
  title={Unpaired multi-modal segmentation via knowledge distillation},
  author={Dou, Qi and Liu, Quande and Heng, Pheng Ann and Glocker, Ben},
  journal={IEEE transactions on medical imaging},
  volume={39},
  number={7},
  pages={2415--2425},
  year={2020},
  publisher={IEEE}
}

@inproceedings{medst2,
  title={Towards cross-modality medical image segmentation with online mutual knowledge distillation},
  author={Li, Kang and Yu, Lequan and Wang, Shujun and Heng, Pheng-Ann},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={34},
  number={01},
  pages={775--783},
  year={2020}
}

@inproceedings{medst3,
  title={Knowledge distillation from multi-modal to mono-modal segmentation networks},
  author={Hu, Minhao and Maillard, Matthis and Zhang, Ya and Ciceri, Tommaso and La Barbera, Giammarco and Bloch, Isabelle and Gori, Pietro},
  booktitle={International Conference on Medical Image Computing and Computer-Assisted Intervention},
  pages={772--781},
  year={2020},
  organization={Springer}
}

@inproceedings{medst_classification,
  title={Variational Knowledge Distillation for Disease Classification in Chest X-Rays},
  author={Sonsbeek, Tom van and Zhen, Xiantong and Worring, Marcel and Shao, Ling},
  booktitle={International Conference on Information Processing in Medical Imaging},
  pages={334--345},
  year={2021},
  organization={Springer}
}

@article{imagetranslation1,
  title={A review on medical imaging synthesis using deep learning and its clinical applications},
  author={Wang, Tonghe and Lei, Yang and Fu, Yabo and Wynne, Jacob F and Curran, Walter J and Liu, Tian and Yang, Xiaofeng},
  journal={Journal of applied clinical medical physics},
  volume={22},
  number={1},
  pages={11--36},
  year={2021},
  publisher={Wiley Online Library}
}

@article{imagetranslation2,
  title={A state-of-the-art review on image synthesis with generative adversarial networks},
  author={Wang, Lei and Chen, Wei and Yang, Wenjia and Bi, Fangming and Yu, Fei Richard},
  journal={IEEE Access},
  volume={8},
  pages={63514--63537},
  year={2020},
  publisher={IEEE}
}


